BETS: The dangers of selection bias in early analyses of the coronavirus disease (COVID-19) pandemic

The coronavirus disease 2019 (COVID-19) has quickly grown from a regional outbreak in Wuhan, China to a global pandemic. Early estimates of the epidemic growth and incubation period of COVID-19 may have been biased due to sample selection. Using detailed case reports from 14 locations in and outside mainland China, we obtained 378 Wuhan-exported cases who left Wuhan before an abrupt travel quarantine. We developed a generative model we call BETS for four key epidemiological events---Beginning of exposure, End of exposure, time of Transmission, and time of Symptom onset (BETS)---and derived explicit formulas to correct for the sample selection. We gave a detailed illustration of why some early and highly influential analyses of the COVID-19 pandemic were severely biased. All our analyses, regardless of which subsample and model were being used, point to an epidemic doubling time of 2 to 2.5 days during the early outbreak in Wuhan. A Bayesian nonparametric analysis further suggests that about 5% of the symptomatic cases may not develop symptoms within 14 days of infection and that men may be much more likely than women to develop symptoms within 2 days of infection.

==> summary.tex <==
\nobibliography*

We find several forms of selection bias in some high-impact early
analyses of the COVID-19 pandemic:

\begin{itemize}
\item Estimation of the initial epidemic growth:
  \begin{enumerate}
  \item Wu, J. T.\ et al.\ \emph{Lancet}, 395(10225),
    2020. PubMed: 32014114.
  \end{enumerate}
\item Estimation of the incubation period:
  \begin{enumerate}[resume]
  \item Backer, J. A.\ et al.\ \emph{Eurosurveillance}, 25(5),
    2020. PubMed: 32046819.
  \item Lauer, S. A.\ et al.\ \emph{Annals of Internal Medicine},
    2020. PubMed: 32150748.
  \item Linton, N. M.\ et al.\ \emph{Journal of Clinical Medicine},
    9(2), 2020. PubMed: 32079150.
  \end{enumerate}
\end{itemize}

We believe the same biases may widely occur in other studies
that \emph{use cases exported from Wuhan and other centers of the
  outbreak} to estimate the epidemic growth, incubation period,
and other epidemiological parameters such as the serial interval
\citep{du2020serial,nishiura2020serial} and parameters related to
disease progression \citep{dorigatti2020report}. \revv{A summary of
  the various types of potential biases in COVID-19 studies can be found in
  \Cref{tab:summary-bias}.} We thus recommend
extreme caution when using the estimated parameters from these studies
when making forecasts about COVID-19.

The first form of selection bias, which we believe is the least
acknowledged in the current literature, arises from travel
restrictions. On January 23, 2020, the government of Wuhan implemented
an abrupt travel quarantine. This policy has a strong
selection effect on the COVID-19 cases who were infected in Wuhan but
confirmed elsewhere. Intuitively, a patient who was infected in
Wuhan on January 22 is much less likely to be observed in the
Wuhan-exported sample than a patient infected on January 15, because
the first patient only has a one-day window to leave Wuhan.

The above heuristic is formalized in this paper. Let $\mathcal{P}$
denote the susceptible population in Wuhan, $\mathcal{D}$ denote
the population of Wuhan-exported cases used in many early analyses,
and $T$ denote the time of contracting the virus. In epidemic modeling, it is
common to assume the density of $T$ is growing exponentially during
the early outbreak: $f_T(t \mid \mathcal{P}) \propto \exp(rt)$, where the
notation $f(\cdot \mid \mathcal{P})$ means the density is among the
general population $\mathcal{P}$.
However, the distribution of $T$ in the Wuhan-exported sample
$\mathcal{D}$ behaves very differently. In an early February preprint
\citep{zhao2020analysis}, we interpreted the above heuristic as the
following density among the Wuhan-exported cases,
\[
  f_T(t \mid \mathcal{D}) \propto (L - t) \exp(rt) \cdot 1_{\{t \le L\}},
\]
where $L$ is the time of the travel quarantine and $1_{\{\cdot\}}$ is the
indicator function. The linear term $(L-t)$ captures the selection due
to the travel quarantine. In \Cref{prop:marginal-s} below, we give a
rigorous proof for this heuristic under a generative model for the
epidemic.

Many early analyses of COVID-19 relied on the assumption that the
density of symptom onset was growing exponentially during the early
outbreak. Let $S$ be the time of symptom onset. The significance of
the above result is that although the exponential growth assumption
\[
  f_S(s \mid \mathcal{P}) \propto \exp(rs)
\]
may be very close to the truth in the general population $\mathcal{P}$, it is
inappropriate for the Wuhan-exported cases $\mathcal{D}$. In
\Cref{prop:marginal-s} below, we derive the following approximation
\[
  f_S(s \mid \mathcal{D}) \propto \exp(rs) \cdot \Big(L +
  \frac{\alpha}{\beta+r} - s \Big)~\text{for}~s \le L,
\]
by assuming the incubation period of COVID-19 follows a
$\text{Gamma}(\alpha,\beta)$ distribution. Furthermore, after reaching
its peak, $f_S(s \mid \mathcal{D})$ diminishes rapidly as $s$
increases. This theoretical result is strongly supported by empirical
data (\Cref{fig:s-marginal}). We believe it is the confusion of $f_S(s
\mid \mathcal{D})$ with $f_S(s \mid \mathcal{P})$ (i.e.\ ignoring the
selection effect of travel quarantine) that led to the
drastic over-estimation of the doubling time of COVID-19 in
Wu et al.\ \citep{wu2020nowcasting} (see
\Cref{sec:estim-epid-growth}).

The second and third forms of selection bias occur in early studies of
the incubation period. Three previous studies only used Wuhan-exported
cases confirmed before the end of January
\citep{backer2020incubation,lauer2020incubation,linton2020incubation}. This
would miss about 30\% of the Wuhan-exported cases that are eventually
confirmed in our dataset, thus leading to serious under-estimation of the
incubation period. The other form of bias is that these studies all
used a likelihood function derived previously that assume the density
of infection time is uniform over the cases' exposure period
\citep{reich2009estimating}. This is a very poor approximation to the
truth as a typical person in Wuhan would have much higher chance of
infection on January 15 than January 22. Failing to account for the
rapid growth of COVID-19 leads to substantial over-estimation of its
incubation period.

These potential biases were mentioned in the limitations of the
previous studies, but no solution was given. In
\Cref{sec:estim-incub-peri} below, we derive explicit
likelihood functions that account for both the \revv{right-truncation} and
epidemic growth for estimating the incubation period. In a
retrospective analysis of our dataset at different time, we observe
the startling effects of both biases if the incorrect
likelihood functions are used (\Cref{fig:ascertainment}). Although the two
biases are in the opposite directions and appear to be balanced out to
some degree in the previous studies, it is evident that the conclusions of these
studies are unreliable and should not be used to \revv{guide health}
policies.

\clearpage

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

